On Giant's Shoulders: Effortless Weak to Strong by Dynamic Logits Fusion

Efficient fine-tuning of large language models for task-specific applications is imperative, yet the vast number of parameters in these models makes their training increasingly challenging. Despite numerous proposals for effective methods, a substantial memory overhead remains for gradient computations during updates. \thm{Can we fine-tune a series of task-specific small models and transfer their knowledge directly to a much larger model without additional training?} In this paper, we explore weak-to-strong specialization using logit arithmetic, facilitating a direct answer to this question. Existing weak-to-strong methods often employ a static knowledge transfer ratio and a single small model for transferring complex knowledge, which leads to suboptimal performance. % To address this, To surmount these limitations, we propose a dynamic logit fusion approach that works with a series of task-specific small models, each specialized in a different task. This method adaptively allocates weights among these models at each decoding step, learning the weights through Kullback-Leibler divergence constrained optimization problems. We conduct extensive experiments across various benchmarks in both single-task and multi-task settings, achieving leading results. By transferring expertise from the 7B model to the 13B model, our method closes the performance gap by 96.4\% in single-task scenarios and by 86.3\% in multi-task scenarios compared to full fine-tuning of the 13B model. Notably, we achieve surpassing performance on unseen tasks. Moreover, we further demonstrate that our method can effortlessly integrate in-context learning for single tasks and task arithmetic for multi-task scenarios.

==> tables/icl.tex <==
\begin{table}[!ht]
\centering
\caption{VS In-context Learning}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}}              &  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{from}}}            & \multicolumn{1}{c}{\textbf{GSM8K }}                   & \multicolumn{1}{c}{\textbf{TruthfulQA }}           & \multicolumn{1}{c}{\textbf{TriviaQA }}  & \multicolumn{1}{c}{\textbf{CNN/DM }}       & \multicolumn{1}{c}{\textbf{MMLU}} \\ 
\multicolumn{1}{c}{}                                             &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{(EM.)}} & \multicolumn{1}{c}{\textbf{(Acc.) }}           & \multicolumn{1}{c}{\textbf{(EM.) }}  & \multicolumn{1}{c}{\textbf{(Rouge 2.) }}       & \multicolumn{1}{c}{\textbf{(Acc.)}} \\  \midrule
\textbf{Base (untuned) }                                          &\textbackslash{}                   & 6.90                   & 46.13                  &       36.44               & 8.94 & 50.07 \\
\textbf{Full Finetune  }                                          &\textbackslash{}                   &   47.23                     &  61.93                      &     56.36                 & 15.50 &  57.94     \\
\textbf{LoRA Tuning }                                             &\textbackslash{}                   &  41.54                      & \textbackslash{}       & 61.89     & 15.27 & 57.15      \\

\textbf{In Context Learning (5-shot)}                                     &\textbackslash{}                   &     20.09                   &  35.12                      &  61.97                    & 9.03 &  53.72      \\
\textbf{Ours}                                                     &1.1b                & 17.36                  & 39.02                  &    50.51             &   13.82    &  48.32\\ 
\textbf{Ours (5-shot)}                                                     &1.1b                &                   &                   &                 &       &  \\ 
\textbf{Ours}                                                     &7b                      & 39.34                  & 61.20                  &      57.11           &   15.36    & 57.14 \\
\textbf{Ours (5-shot)}                                                     &7b                      &  40.03                 &  60.95                 &   62.63              &  12.31    & 57.75 \\\midrule
\end{tabular}
}

\label{tab:icl}
\end{table}
